Low-depth arithmetic circuit lower bounds via shifted partials

We prove super-polynomial lower bounds for low-depth arithmetic circuits using the shifted partials measure [Gupta-Kamath-Kayal-Saptharishi, CCC 2013], [Kayal, ECCC 2012] and the affine projections of partials measure [Garg-Kayal-Saha, FOCS 2020], [Kayal-Nair-Saha, STACS 2016]. The recent breakthrough work of Limaye, Srinivasan and Tavenas [FOCS 2021] proved these lower bounds by proving lower bounds for low-depth set-multilinear circuits. An interesting aspect of our proof is that it does not require conversion of a circuit to a set-multilinear circuit, nor does it involve a random restriction. We are able to upper bound the measures for homogeneous formulas directly, without going via set-multilinearity. Our lower bounds hold for the iterated matrix multiplication as well as the Nisan-Wigderson design polynomials. We also define a subclass of homogeneous formulas which we call unique parse tree (UPT) formulas, and prove superpolynomial lower bounds for these. This generalizes the superpolynomial lower bounds for regular formulas in [Kayal-Saha-Saptharishi, STOC 2014], [Fournier-Limaye-Malod-Srinivasan, STOC 2014].

==> scratch_pad.tex <==
%@article{lst1,
%  author    = {Nutan Limaye and
%               Srikanth Srinivasan and
%               S{\'{e}}bastien Tavenas},
%  title     = {Superpolynomial Lower Bounds Against Low-Depth Algebraic Circuits},
%  booktitle = {Foundations of Computer Science, {FOCS} 2021},
%  pages     = {804--814},
%  publisher = {{IEEE}},
%  year      = {2021},
%  bibsource = {dblp computer science bibliography, https://dblp.org}
%}

%@article{lst2,
%  author    = {Nutan Limaye and
%               Srikanth Srinivasan and
%               S{\'{e}}bastien Tavenas},
%  title     = {{New Non-FPT Lower Bounds for Some Arithmetic Formulas}},
%  journal   = {Electron. Colloquium Comput. Complex.},
%  pages     = {94},
%  year      = {2021},
%  url       = {https://eccc.weizmann.ac.il/report/2021/094},
%  bibsource = {dblp computer science bibliography, https://dblp.org}
%}

*******************************************************

% \begin{theorem}
% 	Let $n, \Delta$, and $d$ be integers such that $n \geq \alert{10}$ and $d \leq \log n$. Then, there exists an explicit polynomial $f_{n, d, \Delta}$ such that any homogeneous arithmetic formula of product-depth $\Delta$ computing $f_{n, d, \Delta}$ has size $\lb$.
% \end{theorem}

% \noindent Let $C = T_1 + \cdots + T_s$ be a homogeneous arithmetic formula of product-depth $\Delta$, where $T_i = \sum_{i \in [s]} Q_{i, 1}\cdots Q_{i, t_i}$ and for all $j \in [t_i]$, $Q_{i, j}$ is a homogeneous polynomial of degree $d_{i,j}$. We shall first obtain an upper bound on $\SP_{k, \ell}(C)$. Because of the sub-additivity of $\SP_{k, \ell}$, it is sufficient to obtain an upper bound on $\SP_{k, \ell}(T_i)$ for all $i \in [s]$ For a fixed $i$, it follows from Lemma \ref{lem:der-structure} that 
% \begin{align*}
% 	\spacespanned{\vecx^{\ell}\partial^k\paren{T_i}} \subseteq \sum \limits_{\substack{S \subseteq [t_i], \ k_0, \ell_0 \in [0..k] \\ k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \entropy_k(d_1, \cdots, d_{t_i})/2}} \spacespanned{ \vecx^{\ell + \ell_0}\cdot\partial^{k_0}\paren{\prod_{j\in S} Q_{i,j}}}.
% \end{align*}
% Thus, 
% \begin{align*}
% 	\SP_{k, \ell}\paren{T_i} &= \dim \spacespanned{\vecx^{\ell}\partial^k T_i} \\
% 	&\leq 2^{t_i}\cdot k^2 \cdot \max \limits_{\substack{S \subseteq [t_i], \ k_0, \ell_0 \in [0..k] \\ k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \entropy_k(d_1, \cdots, d_{t_i})/2}} \dim\spacespanned{ \vecx^{\ell + \ell_0}\cdot\partial^{k_0}\paren{\prod_{j\in S} Q_{i,j}}} \\
% 	&= 2^{t_i}\cdot k^2 \cdot \max \limits_{\substack{\ k_0, \ell_0 \in [0..k] \\ k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \entropy_k(d_1, \cdots, d_{t_i})/2}} M(n, k_0)\cdot M(n, \ell + \ell_0) \\
% 	&\leq 2\cdot 2^d \cdot \max \limits_{\substack{\ k_0, \ell_0 \in [0..k] \\ k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \entropy_k(d_1, \cdots, d_{t_i})/2}} M(n, k_0)\cdot M(n, \ell + \ell_0).
% \end{align*}
% Hence, 
% \begin{align*}
% 	\SP_{k, \ell}\paren{C} \leq s\cdot 2\cdot 2^d \cdot \max \limits_{\substack{\ k_0, \ell_0 \in [0..k] \\ k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \entropy_k(d_1, \cdots, d_{t_i})/2}} M(n, k_0)\cdot M(n, \ell + \ell_0).
% \end{align*}
% Suppose that the maximum of the above expression is at $k_0 = k_0^*$ and $\ell_0 = \ell_0^*$. Then,
% \begin{align*}
% 	\paren{C} \leq s\cdot 2\cdot 2^d \cdot M(n, k_0^*)\cdot M(n, \ell + \ell_0^*)
% \end{align*}
% and $k_0^*, \ell_0^* \in [k], \ k_0^* + \frac{k}{d-k}\cdot \ell_0^* \leq k - \frac{\entropy_k(d_1, \cdots, d_{t_i})}{2}$.

% The following lemma proved in Appendix \alert{??} gives a lower bound on $\SP_{k, \ell}$ for an explicit polynomial.
% \begin{lemma}\label{lem:lb_SP_NW}
% 		Let $n, \Delta$, and $d$ be integers such that $n \geq \alert{10}$ and $d \leq \log n$. Then, there exists an explicit polynomial $f_{n, d, \Delta}$ such that $\SP_{k, \ell}(f_{n, d, \Delta}) \geq \frac{1}{2}\cdot\paren{\frac{n}{d}}^k\cdot M(n, \ell)$.
% \end{lemma}
% \noindent Thus, for any formula $C$ computing $f_{n, d, \Delta}$, we have 
% \begin{align} 
% 	s &\geq \frac{\frac{1}{2}\cdot\paren{\frac{n}{d}}^k\cdot M(n, \ell)}{2\cdot 2^d \cdot M(n, k_0^*)\cdot M(n, \ell + \ell_0^*)} \nonumber \\
% 	&= \frac{1}{2^{O(d)}}\cdot \frac{\paren{\frac{n}{d}}^k}{M(n, k_0^*)} \cdot \frac{M(n, \ell)}{M(n, \ell + \ell_0^*)}. 
% \end{align} \label{eqn:low_depth_lb_calculation_1}
% \begin{observation} \label{obs:comparing_M(n,l)_M(n,l+D2)}
% 	$\frac{M(n, \ell)}{M(n, \ell + \ell_0^*)} = \paren{1 - o(1)}\cdot \paren{\frac{\ell}{n}}^{\ell_0^*}$.
% \end{observation}
% \begin{proof}
% 	\begin{flalign*}
% 		&& \frac{M(n, \ell)}{M(n, \ell + \ell_0^*)} &= \frac{{n + \ell - 1 \choose \ell}}{{n + \ell + \ell_0^* - 1 \choose \ell + \ell_0^*}} \\
% 		&& &= \frac{\frac{(n + \ell - 1)!}{(n - 1)!\ \ell!}}{\frac{(n + \ell + \ell_0^* - 1)!}{(n - 1)!\ (\ell + \ell_0^*)!}} \\
% 		&& &= \frac{(\ell + \ell_0^*)(\ell + \ell_0^* - 1)(\ell + \ell_0^* - 2)\cdots (\ell + 1)}{(n + \ell + \ell_0^* - 1)(n + \ell + \ell_0^* - 2)(n + \ell + \ell_0^* - 3)\cdots (n + \ell)} \\
% 		&& &= \frac{1}{\Big(\frac{n-1}{\ell + \ell_0^*} + 1\Big) \Big(\frac{n-1}{\ell + \ell_0^* - 1} + 1 \Big) \Big(\frac{n-1}{\ell + \ell_0^* - 2} + 1\Big) \cdots \Big(\frac{n-1}{\ell + 1} + 1\Big) } \\
% 		&& &\geq \frac{1}{\paren{\frac{n}{\ell} + 1}^{\ell_0^*}} \\
% 		&& &= \paren{1 - o(1)}\cdot \paren{\frac{\ell}{n}}^{\ell_0^*} && \paren{\text{as } \ell = o(n)}.
% 	\end{flalign*}
% \end{proof}
% \noindent Thus, from Equation \eqref{eqn:low_depth_lb_calculation_1}
% \begin{flalign*}
% 	&& s &\geq \frac{1}{2^{O(d)}} \cdot \frac{\paren{\frac{n}{d}}^k}{\paren{\frac{e(n + k_0^* - 1)}{k_0^*}}^{k_0^*}} \cdot \paren{1 - o(1)}\cdot \paren{\frac{\ell}{n}}^{\ell_0^*} \\
% 	&& &= \frac{1}{2^{O(d)}} \cdot \frac{\paren{\frac{n}{d}}^k}{\paren{\frac{n}{k_0^*}}^{k_0^*}}\cdot\paren{\frac{\ell}{n}}^{\ell_0^*} && \paren{\text{because } k_0^* \leq k = o(n)} \\
% 	&& &\geq \frac{1}{d^{O(d)}} \cdot \frac{n^k}{n^{k_0^*}}\cdot \paren{\frac{n^{\frac{k}{d-k}}}{n}}^{\ell_0^*} && \paren{\text{because } k \leq d} \\
% 	&& &\geq \frac{1}{d^{O(d)}} \cdot n^{k - k_0^* + \frac{k}{d - k}\cdot \ell_0^*}\\
% 	&& &\geq \frac{1}{d^{O(d)}} \cdot n^\frac{\entropy_k(d_1, \cdots, d_{t_i})}{2} && \paren{\text{as } k_0^* + \frac{k}{d - k}\cdot \ell_0^* \leq k - \frac{\entropy_k(d_1, \cdots, d_{t_i})}{2}}.
% \end{flalign*}%\label{eqn:low_depth_lb_calculation_2}

*****************************

Note that $d,k,r = o(qd)$. Also, observe that because $\ell = \floor{\frac{q d^2}{n_0}}$ and $n_0 = 2(d-k)\cdot \paren{\frac{q d}{k}}^\frac{k}{d-k}$,
    \begin{flalign*}
        && \ell &\leq \frac{q d^2}{2c(d-k)}\paren{\frac{k}{q d}}^\frac{k}{d-k} \\
        && &\leq \frac{q d^2}{2c(d-k)}\paren{\frac{k}{q d}}^\frac{1}{29} && \paren{\text{because } k \in \brac{\frac{d}{30}, \frac{d}{2}}} \\
        && &= \frac{d k^\frac{1}{29}}{2c(d-k)}{(qd)^\frac{28}{29}} \\
        && &= o(qd).
    \end{flalign*}
    Moreover, $\ell \geq (1-o(1))\frac{qd^2}{n_0}\geq \frac{(1-o(1))q d^2}{2(d-k)}\paren{\frac{k}{qd}}^\frac{k}{d-k} = O\paren{qd\paren{\frac{k}{qd}}^\frac{k}{d-k}} \geq O\paren{(qd)^\frac{1}{30}}$ as $k \in \brac{\frac{d}{30}, \frac{d}{2}}$. Thus, $d,k,r = o(\ell)$. Hence, form \eqref{eqn:clm_C_1_intermediate},
    \begin{align*}
        \frac{\chi(r+1)}{\chi(r)}  &\leq \frac{d}{q} \cdot\frac{(1+o(1))qd}{(1-o(1))\ell}\\ 
        &= o(1),
    \end{align*}
    because $d^2 = o(\ell)$.

****************************************


    \begin{flalign*}
        && \ell &\geq \frac{qd^2}{n_0} - 1\\
        && &= \frac{qd^2}{2(d-k)}\paren{\frac{k}{qd}}^{\frac{k}{d-k}} - 1 \\
        && &\geq  \frac{qd^2}{2(d-k)}\paren{\frac{k}{qd}}^{\frac{d/2 - \sqrt{d}/8}{d/2 + \sqrt{d}/8}} - 1 && \paren{\text{because $k = o(qd)$ and $k\leq \frac{d}{2} - \frac{\sqrt{d}}{8}$}}\\
        && &= \frac{qd^2}{2(d-k)}\paren{\frac{k}{qd}}^{1 - \frac{\sqrt{d}/4}{d/2 + \sqrt{d}/8}} - 1\\
        && &=  \frac{qd^2}{2(d-k)}\cdot \frac{k}{qd}\cdot \paren{\frac{qd}{k}}^{\frac{2}{4\sqrt{d} + 1}} - 1\\ 
        && &= \frac{dk}{2(d-k)}\paren{\frac{qd}{k}}^{\frac{1}{3\sqrt{d}}} - 1 \\
        && &\geq \frac{(qd)^\frac{1}{3\sqrt{d}}}{2} - 1 \\
        && &= \frac{2^\frac{\log qd}{3\sqrt{d}}}{2} - 1.
    \end{flalign*}
As $d \leq \log^{2-\epsilon}n$ and $qd \geq \frac{n}{4}$, $\frac{\log qd}{3\sqrt{d}} \geq \frac{\log^{\epsilon/2}n}{4} = \omega(4 \log \log n)$. As $4 \log \log n \geq \log d^2$, $\ell = o(d^2)$.

********************************************

\begin{lemma}[{\bf $P_\vecw$ as a hard polynomial}]
	For integers $h,d > 100$ such that $d < 2^{h/60}$ , and any parameter $k \in \brac{\frac{d}{30}, \frac{d}{2}}$, there exists an $h$\unbiased~word $\vecw \in [-h..h]^d$, integers $n_0 \le n$, $\ell=\floor{\frac{n\cdot d}{n_0}}$ such that $n_0 \approx 2(d-k)\!\cdot\! \paren{{\frac{n}{k}}}^{\frac{k}{d-k}}$ and the following bounds hold. Here $n$ refers to the number of variables in $P_{\vecw}$, i.e., $n=\sum_{i \in [d]} 2^{\abs{w_i}}$.
	\begin{enumerate}
	    \item $\SP_{k,\ell}(P_{\vecw}) \ge 2^{-O(d)}\!\cdot\! M(n,k)\!\cdot\! M(n,\ell)$,
	    \item $\APP_{k,n_0}(P_{\vecw}) \ge 2^{-O(d)}\!\cdot\! M(n,k)$.
	\end{enumerate}
	\label{lem:hard-poly}
\end{lemma}

************************************************************

%\begin{align*}
%\Lambda &= \frac{M(n,k)\!\cdot\! M(n,\ell)}{\max_{k_0 + \frac{k}{d-k}\cdot\ell_0 \le k - \gamma}M(n,k_0)\!\cdot\! M(n,\ell+\ell_0)} = \frac{M(n,\ell + d - k)\!\cdot\! M(n,\ell)}{\max_{k_0 + \frac{k}{d-k}\cdot\ell_0 \le k - \gamma}M(n,k_0)\!\cdot\! M(n,\ell+\ell_0)} \\ &= \min_{k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \gamma}\frac{M(n,k)\!\cdot\! M(n,\ell)}{M(n,k_0)\!\cdot\! M(n,\ell+\ell_0)} \qquad = \min_{k_0 + \frac{k}{d-k}\cdot \ell_0 \le k - \gamma}\frac{M(n,\ell + d - k)}{M(n,k_0)\!\cdot\! M(n,\ell+\ell_0)} \numberthis
%\label{eqn:best-lb-2}
%\end{align*}

**********************************************************

\begin{flalign*}
    && s &\geq \frac{\binom{n}{k}}{\binom{n_0 + dk - k}{n_0}} \\
    && &\geq \frac{\paren{\frac{n}{k}}^k}{\paren{\frac{e(n_0 + kd-k))}{n_0}}^{n_0}} \\
    && &= \frac{\paren{\frac{n}{k}}^k}{\paren{\frac{e(kd + 1)}{k+1}}^{k+1}} && \text{(as $n_0 = k+1$)}\\
    && &\geq \frac{1}{n^{O(1)}}\frac{\paren{\frac{n}{k}}^k}{\paren{\frac{e + n/4}{n/4ed}}^{k}} && \paren{\text{as $k = \floor{\frac{n}{4ed}}$}}\\
    && &= \frac{1}{n^{O(1)}}\paren{\frac{n}{ked}}^k \\
    && &\geq \frac{4^k}{n^{O(1)}} && \text{(as $ked \leq n/4$)} \\
    && &= 2^{\Omega\paren{\frac{n}{d}}}.
\end{flalign*}

****************************************

\newpage
	\tableofcontents {\protect\thispagestyle{empty}}
	\newpage
	\pagenumbering{arabic}
	

==> sec_discussion.tex <==
%!TeX spellcheck = en_GB
\section{Few problems}
To be added...

==> sec_overview.tex <==
\newcommand{\linmaps}[1]{\mathcal{#1}}

\section{Proof overview} \label{sec:overview}
At a high level, the proof outline for our lower bound  in theorem \ref{thm:upt} looks similar to that of (the simplified versions of) the known lower bounds. Let $f(\vecx)$ be a homogeneous $n$-variate polynomial of degree $d$. \\

\noindent {\bf Step 1: depth reduction.} One first shows that if $f(\vecx)$ is computed by a {\em small} circuit from some restricted subclass of circuits, then there is a corresponding subclass of depth four circuits such that $f(\vecx)$ is also computed by a {\em relatively small} from this subclass\footnote{
   Some major results in the area such as \cite{Raz03, lst1} did not originally proceed via a depth reduction but instead analysed formulas directly. These results can however be restated as first doing a depth reduction and then applying the appropriate measure. 
}. We apply the usual depth reduction Specifically, we observe that :

\begin{lemma}\label{upt:depthReduction}
    {\bf Depth Reduction for UPT formulas.}
    Let $f(\vecx) \in \F[\vecx]$ be a polynomial computed by a 
\end{lemma}


\noindent {\bf Step 2: employing a suitable set of linear maps.}
    Let $\F[\vecx]^{=d}$ be the vector space of homogeneous polynomials of degree $d$, 
    $W$ be a suitable vector space and $\mathrm{Lin}(\F[\vecx]^{=d}, W)$ be the space of linear maps from $\F[\vecx]^{=d}$  to $W$. Let $\linmaps{L} \subseteq \mathrm{Lin}(\F[\vecx]^{=d}, W)$ be a suitably chosen subspace of linear maps. 
    The complexity measure corresponding to such a collection of linear maps $\linmaps{L}$
    is 
        $$ \dim(\linmaps{L} \cdot f), \quad \text{where~} \linmaps{L} \cdot f \defeq \left\{ L \cdot f \ : \ L \in \linmaps{L} \right\}. $$
    A long line of works initiated by \cite{}, with culminating in \cite{lst1, lst2} employ maps corresponding to {\em partial evaluations} and use that to show lower bounds for various models including multilinear formulas \cite{raz}.
    In this work, we analyze the set of maps known as {\em shifted partials}. Let $k, \ell \geq 0$ be two integers and $\vecalpha, \vecbeta \in \Z_{\geq 0}^n $ be two multisets of size $k, \ell$ respectively. The corresponding shifted partial map  
        $$ \vecx^{\vecbeta} \cdot \partialf^{\vecalpha} : \F[\vecx]^{=d} \mapsto \F[\vecx]^{=(d-k+\ell)} \quad \text{is defined as~}(\vecx^{\vecbeta} \cdot \partialf^{\vecalpha}) \cdot f  = \vecx^{\vecbeta} \cdot (\partialf^{\vecalpha} f ). $$
    The corresponding complexity measure denoted $\SP_{k, \ell} $ is:
        $$ \SP_{k,\ell}(f) := \dim \langle \vecx^\ell.\partialf^k (f) \rangle. $$
    Our main insight is that $\SP_{k,\ell}$ is {\em relatively small} for a product of polynomials. 
    \begin{lemma}(informal version of lemma \ref{lem:spub})
        Let $T(\vecx) \in \F[\vecx]^{=d}$ be a product of polynomials, i.e. $T = Q_1(\vecx) \cdot Q_2(\vecx) \cdot \ldots \cdot Q_t(\vecx)$, where $\deg(Q_i) = d_i$ and $d = \sum_{i \in [t]} d_i$. Then for $k \geq 1$, there exists a suitable choice of $\ell$
        such that
        \begin{eqnarray*}
            \SP_{k,\ell}(T) & \lessapprox & \frac{k^k}{n^{\gamma(k)}} \cdot \min \left( \binom{n+k-1}{k} \cdot \binom{n+\ell-1}{\ell}, \binom{n+d-k+\ell-1}{d-k+\ell} \right), \text{where~}\\
            \gamma(k) & \defeq & \min_{\stackrel{(k_1, k_2, \ldots, k_t) :}{ k_1 + k_2 + \ldots + k_t = k}}{\quad \sum_{i \in [t]} \abs{k_i - \frac{k d_i}{d}}}    
        \end{eqnarray*}
    \end{lemma}
\noindent Note that $\SP_{k,\ell}(T)$ is trivially upper bounded by 
    $\min \left( \binom{n+k-1}{k} \cdot \binom{n+\ell-1}{\ell}, \binom{n+d-k+\ell-1}{d-k+\ell} \right)$
    so that the {\em gain} is approximately a factor of $\frac{n^{\gamma(k)}}{k^k} $. \\
    
\noindent {\bf Step 3: lower bounding the measure for an explicit polynomial.} We now show that for some explicit polynomial $f(\vecx)$, the measure is suitably large. From this we conclude that $f(\vecx)$ cannot have small UPT formulas.




